Neural Image Compression with Text-guided Encoding for both Pixel-level and Perceptual Fidelity

Recent advances in text-guided image compression have shown great potential to enhance the perceptual quality of reconstructed images. These methods, however, tend to have significantly degraded pixel-wise fidelity, limiting their practicality. To fill this gap, we develop a new text-guided image compression algorithm that achieves both high perceptual and pixel-wise fidelity. In particular, we propose a compression framework that leverages text information mainly by text-adaptive encoding and training with joint image-text loss. By doing so, we avoid decoding based on text-guided generative models -- known for high generative diversity -- and effectively utilize the semantic information of text at a global level. Experimental results on various datasets show that our method can achieve high pixel-level and perceptual quality, with either human- or machine-generated captions. In particular, our method outperforms all baselines in terms of LPIPS, with some room for even more improvements when we use more carefully generated captions.

==> assets/tables/low_high_res_encoding_time.tex <==
\begin{table}[t]
\caption{\camera{\textbf{Computational cost of high-resolution image.} We compare the encoding speed of a low-resolution image (256x256, `Low' in the table) and a high-resolution image (1788x2641, `High' in the table). Compared with the base model, ELIC, we observe that the relative slowdown grows smaller as we consider a higher resolution (+10.2\% $\rightarrow$ +4.8\%). }} 

\label{tab:low_high_res_comparison}
\begin{center}
\begin{small}
\begin{tabular}{lrrr}
    \toprule
     & Encoding@Low (ms) & Encoding@High (ms)\\
    \midrule
    LIC-TCM & 112.07 & 960.09 \\
    MS-ILLM & 70.39 & 800.45 \\
    ELIC & 71.35 & 793.41 \\
    \midrule
    \textbf{TACO} & 78.60 (+10.2\%) & 832.07 (+4.8\%) \\
    \bottomrule
\end{tabular}
\end{small}
\end{center}
\end{table}


==> assets/tables/where_to_input_text.tex <==
\begin{table}[t]
\caption{{\color{red}change to CLIC} \student{\textbf{Ablation: Encoder-only strategy.} Performance comparison based on where input the text at a specific point. We add the text adapter whether at encoding(our approach), decoding(proposed approach in \citep{qin_comp_23}), all(proposed approach in \citep{tgic}). In this result, we find that using text when encoding is a more effective way.}}
\label{tab:abation-on-input-text}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
    \toprule
     & BPP & LPIPS ↓ & PSNR ↑ & FID ↓ \\
    \midrule
    \makecell[l]{Enc. only} & 0.66 & \textbf{0.013} & \textbf{33.06} & \textbf{0.926}\\
    \makecell[l]{Dec. only} & 0.67 & 0.014 & 32.89 & 0.987\\
    \makecell[l]{Both} & 0.67 & 0.014 & 32.86 & 0.944\\
    \bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table}


==> assets/tex/Ablation_caption_quality_results.tex <==
\begin{figure}[!tb]
    \centerline{\includegraphics[width=\columnwidth]{assets/figures/Ablation_Study/modify-caption-GPT4/modified_GPT4_LPIPS.pdf}} 
    \caption{ {\color{red}replace to non-semantic version} Results about the role of text information in CLIC. We compare the performance between semantic captions(including captions that are highlighted in various aspects) and randomly generated captions. We find that using non-semantic captions contributes the lower performance and adapting variation in captions is not an effective approach for high performance when using TACO.}
    \label{fig:results_based_on_caption_quality} 
\end{figure}

==> assets/tex/Ablation_freezing.tex <==
\begin{figure}[!t]
    \centerline{\includegraphics[width=\columnwidth]{assets/figures/Ablation_Study/freeze_base/Abl_Freeze_LPIPS.pdf}} % 
     \centerline{\includegraphics[width=\columnwidth]{assets/figures/Ablation_Study/freeze_base/Abl_Freeze_PSNR.pdf}}
    \caption{{\color{red}change to CLIC result - move to Appendix }Comparison result between training from scratch and training only text adapter while freezing the baseline.}
    \label{fig:model_freezing} 
\end{figure}

==> assets/tex/Ablation_loss_coeff.tex <==
\begin{figure}[!t]
    \centerline{\includegraphics[width=\columnwidth]{assets/figures/Ablation_Study/Loss/MSCOCO_coeff_LPIPS.pdf}} % 
    \caption{{\color{red}change to CLIC result - move to Appendix }Ablation results on optimal hyperparameters of LPIPS and joint-image-text loss. We evaluate on MS-COCO 30k using models which are trained on all cases mentioned \cref{ssec:ablations}}
    \label{fig:loss_coefficient_ablation} 
\end{figure}




==> assets/tex/Ablation_unimodal_adapter_archi.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{assets/figures/uni_directional.pdf}
\caption{Uni-directional text adapter.}
\end{figure}

==> assets/tex/Ablation_where_to_use_text_result.tex <==
\begin{figure}[!t]
    %\centerline{\includegraphics[]{example-image-duck}} % 
    \centerline{\includegraphics[width=\columnwidth]{assets/figures/Ablation_Study/Where_to_input_text/Abl_Input_text_LPIPS.pdf}} % 
    \caption{Ablation: where to use text}
    \label{fig:where_to_use_text} 
\end{figure}

==> assets/tex/caption_result.tex <==
\begin{figure*}[!t]
    % \centerline{\includegraphics[width=\columnwidth]{example-image-duck}} % 
    \centerline{\includegraphics[width=2\columnwidth, height=4.0 cm]{example-image-duck}} % 
    \caption{Visual result : compressed images with other baselines}
    \label{fig:image} 
    
    \centerline{\includegraphics[width=2\columnwidth, height=4.0 cm]{example-image-duck}} % 
    \caption{Caption score result graph : CIDEr, BLEU-4, ...}
    \label{fig:image} 

    %  \centerline{\includegraphics[width=columnwidth, height=3.0 cm]{example-image-duck}} % 
    % \caption{Main result graph : caption scores}
    % \label{fig:text} 
    
\end{figure*}

==> assets/tex/detailed_encoding_figure.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{assets/figures/encoder_detailed.pdf}
\caption{Detailed description of how text adapter work in encoding.}
\label{detail_encoding}
\end{figure}

==> assets/tex/duck.tex <==
\begin{figure}[!t]
    \centerline{\includegraphics[width=\columnwidth]{example-image-duck}} % 
    % \centerline{\includegraphics[width=\columnwidth]{figures/icml_numpapers.pdf}} % 

    \caption{Figure shows image compression ruins the Text-semantic information}
    \label{fig:duckduck} 
\end{figure}


==> assets/tex/prompt_for_caption_generation.tex <==

\texttt{\\ You are part of a team of bots that generate captions. You work with a reconstruction bot that will reconstruct images from the compressed image's bitstream and caption. For example, if we have the bitstream by compressing the image of the forest, outputting "a beautiful morning in the woods with the sun peaking through the trees" will trigger your partner to reconstruct an image of the forest morning from the compressed bitstream and the generated caption. You will prompted by people looking to reconstruct like original image. The way to accomplish this is to generate descriptive captions that describe the information of images. \\\\ There are a few rules to follow: \\\\  - You will only ever output a single image description per user request. \\ - Sometimes the user will request that you modify previous captions. In this case, you should refer to your previous conversations with the user and make the modifications requested. \\ - When modifications are requested, you should not simply make the description longer. You should refactor the entire description to integrate the suggestions. \\ - Other times the user will not want modification, but instead want a new image. In this case, you should ignore your previous conversation with the user.\\\\ "Generate the caption of the attached image following the rule mentioned before. Delete the information that can't be recognized visually. Image descriptions must be within 10 words. Extra words will be ignored."}


==> assets/tex/prompt_for_caption_modification.tex <==

\texttt{\\ You are part of a team of bots that generate captions. You work with a reconstruction bot that will reconstruct images from the compressed image's bitstream and caption. For example, if we have the bitstream by compressing the image of the forest, outputting "a beautiful morning in the woods with the sun peaking through the trees" will trigger your partner to reconstruct an image of the forest morning from the compressed bitstream and the generated caption. You will prompted by people looking to reconstruct like original image. The way to accomplish this is to generate descriptive captions that describe the information of images. \\\\ There are a few rules to follow: \\\\  - You will only ever output a single image description per user request. \\ - Sometimes the user will request that you modify previous captions. In this case, you should refer to your previous conversations with the user and make the modifications requested. \\ - When modifications are requested, you should not simply make the description longer. You should refactor the entire description to integrate the suggestions. \\ - Other times the user will not want modification, but instead want a new image. In this case, you should ignore your previous conversation with the user.}


==> assets/tex/rate_distortion_kodak.tex <==
\begin{figure*}[ht]
    \centering
    \begin{subfigure}{.8\textwidth}
        \includegraphics[width=\columnwidth]{assets/figures/metric_kodak/PSNR_Kodak.pdf}
    \end{subfigure}
    
    \begin{subfigure}{.33\textwidth}
        \includegraphics[width=\columnwidth]{assets/figures/metric_kodak/MS-SSIM_Kodak.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.33\textwidth}
        \includegraphics[width=\columnwidth]{assets/figures/metric_kodak/LPIPS_Kodak.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.33\textwidth}
        \includegraphics[width=\columnwidth]{assets/figures/metric_kodak/FID_Kodak.pdf}
    \end{subfigure}
    
    
    \begin{subfigure}{.33\textwidth}
        \includegraphics[width=\columnwidth]{assets/figures/metric_kodak/KID_Kodak.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.33\textwidth}
        \includegraphics[width=\columnwidth]{assets/figures/metric_kodak/NIMA_Kodak.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.33\textwidth}
        \includegraphics[width=\columnwidth]{assets/figures/metric_kodak/IS_Kodak.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.33\textwidth}
        \includegraphics[width=\columnwidth]{assets/figures/metric_kodak/DISTS_Kodak.pdf}
    \end{subfigure}
    % \caption{Comparisons of methods across various distortion and statistical fidelity metrics for the CLIC 2020 test set. Reference models (VTM 19.2, BPG, and No-GAN (Ours)) achieve the best MS-SSIM and PSNR scores, but display poor statistical fidelity as measured by FID and KID. GAN methods (\Ours, \hific, and Multi-Realism) are able to trade some distortion for statistical fidelity. \Ours (Ours) is able to achieve better statistical fidelity as measured by FID and KID vs. HiFiC at equivalent distortion levels.
    % }
    \label{fig:rate_plots}
\end{figure*}


==> sections/0_format.tex <==
All submissions must follow the specified format.

\subsection{Dimensions}




The text of the paper should be formatted in two columns, with an
overall width of 6.75~inches, height of 9.0~inches, and 0.25~inches
between the columns. The left margin should be 0.75~inches and the top
margin 1.0~inch (2.54~cm). The right and bottom margins will depend on
whether you print on US letter or A4 paper, but all final versions
must be produced for US letter size.
Do not write anything on the margins.

The paper body should be set in 10~point type with a vertical spacing
of 11~points. Please use Times typeface throughout the text.

\subsection{Title}

The paper title should be set in 14~point bold type and centered
between two horizontal rules that are 1~point thick, with 1.0~inch
between the top rule and the top edge of the page. Capitalize the
first letter of content words and put the rest of the title in lower
case.

\subsection{Author Information for Submission}
\label{author info}

ICML uses double-blind review, so author information must not appear. If
you are using \LaTeX\/ and the \texttt{icml2023.sty} file, use
\verb+\icmlauthor{...}+ to specify authors and \verb+\icmlaffiliation{...}+ to specify affiliations. (Read the TeX code used to produce this document for an example usage.) The author information
will not be printed unless \texttt{accepted} is passed as an argument to the
style file.
Submissions that include the author information will not
be reviewed.

\subsubsection{Self-Citations}

If you are citing published papers for which you are an author, refer
to yourself in the third person. In particular, do not use phrases
that reveal your identity (e.g., ``in previous work \cite{langley00}, we
have shown \ldots'').

Do not anonymize citations in the reference section. The only exception are manuscripts that are
not yet published (e.g., under submission). If you choose to refer to
such unpublished manuscripts \cite{anonymous}, anonymized copies have
to be submitted
as Supplementary Material via CMT\@. However, keep in mind that an ICML
paper should be self contained and should contain sufficient detail
for the reviewers to evaluate the work. In particular, reviewers are
not required to look at the Supplementary Material when writing their
review (they are not required to look at more than the first $8$ pages of the submitted document).

\subsubsection{Camera-Ready Author Information}
\label{final author}

If a paper is accepted, a final camera-ready copy must be prepared.
%
For camera-ready papers, author information should start 0.3~inches below the
bottom rule surrounding the title. The authors' names should appear in 10~point
bold type, in a row, separated by white space, and centered. Author names should
not be broken across lines. Unbolded superscripted numbers, starting 1, should
be used to refer to affiliations.

Affiliations should be numbered in the order of appearance. A single footnote
block of text should be used to list all the affiliations. (Academic
affiliations should list Department, University, City, State/Region, Country.
Similarly for industrial affiliations.)

Each distinct affiliations should be listed once. If an author has multiple
affiliations, multiple superscripts should be placed after the name, separated
by thin spaces. If the authors would like to highlight equal contribution by
multiple first authors, those authors should have an asterisk placed after their
name in superscript, and the term ``\textsuperscript{*}Equal contribution"
should be placed in the footnote block ahead of the list of affiliations. A
list of corresponding authors and their emails (in the format Full Name
\textless{}email@domain.com\textgreater{}) can follow the list of affiliations.
Ideally only one or two names should be listed.

A sample file with author names is included in the ICML2023 style file
package. Turn on the \texttt{[accepted]} option to the stylefile to
see the names rendered. All of the guidelines above are implemented
by the \LaTeX\ style file.

\subsection{Abstract}

The paper abstract should begin in the left column, 0.4~inches below the final
address. The heading `Abstract' should be centered, bold, and in 11~point type.
The abstract body should use 10~point type, with a vertical spacing of
11~points, and should be indented 0.25~inches more than normal on left-hand and
right-hand margins. Insert 0.4~inches of blank space after the body. Keep your
abstract brief and self-contained, limiting it to one paragraph and roughly 4--6
sentences. Gross violations will require correction at the camera-ready phase.

\subsection{Partitioning the Text}

You should organize your paper into sections and paragraphs to help
readers place a structure on the material and understand its
contributions.

\subsubsection{Sections and Subsections}

Section headings should be numbered, flush left, and set in 11~pt bold
type with the content words capitalized. Leave 0.25~inches of space
before the heading and 0.15~inches after the heading.

Similarly, subsection headings should be numbered, flush left, and set
in 10~pt bold type with the content words capitalized. Leave
0.2~inches of space before the heading and 0.13~inches afterward.

Finally, subsubsection headings should be numbered, flush left, and
set in 10~pt small caps with the content words capitalized. Leave
0.18~inches of space before the heading and 0.1~inches after the
heading.

Please use no more than three levels of headings.

\subsubsection{Paragraphs and Footnotes}

Within each section or subsection, you should further partition the
paper into paragraphs. Do not indent the first line of a given
paragraph, but insert a blank line between succeeding ones.

You can use footnotes\footnote{Footnotes
should be complete sentences.} to provide readers with additional
information about a topic without interrupting the flow of the paper.
Indicate footnotes with a number in the text where the point is most
relevant. Place the footnote in 9~point type at the bottom of the
column in which it appears. Precede the first footnote in a column
with a horizontal rule of 0.8~inches.\footnote{Multiple footnotes can
appear in each column, in the same order as they appear in the text,
but spread them across columns and pages if possible.}

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{figures/icml_numpapers}}
\caption{Historical locations and number of accepted papers for International
Machine Learning Conferences (ICML 1993 -- ICML 2008) and International
Workshops on Machine Learning (ML 1988 -- ML 1992). At the time this figure was
produced, the number of accepted papers for ICML 2008 was unknown and instead
estimated.}
\label{icml-historical}
\end{center}
\vskip -0.2in
\end{figure}

\subsection{Figures}

You may want to include figures in the paper to illustrate
your approach and results. Such artwork should be centered,
legible, and separated from the text. Lines should be dark and at
least 0.5~points thick for purposes of reproduction, and text should
not appear on a gray background.

Label all distinct components of each figure. If the figure takes the
form of a graph, then give a name for each axis and include a legend
that briefly describes each curve. Do not include a title inside the
figure; instead, the caption should serve this function.

Number figures sequentially, placing the figure number and caption
\emph{after} the graphics, with at least 0.1~inches of space before
the caption and 0.1~inches after it, as in
\cref{icml-historical}. The figure caption should be set in
9~point type and centered unless it runs two or more lines, in which
case it should be flush left. You may float figures to the top or
bottom of a column, and you may set wide figures across both columns
(use the environment \texttt{figure*} in \LaTeX). Always place
two-column figures at the top or bottom of the page.

\subsection{Algorithms}

If you are using \LaTeX, please use the ``algorithm'' and ``algorithmic''
environments to format pseudocode. These require
the corresponding stylefiles, algorithm.sty and
algorithmic.sty, which are supplied with this package.
\cref{alg:example} shows an example.

\begin{algorithm}[tb]
   \caption{Bubble Sort}
   \label{alg:example}
\begin{algorithmic}
   \STATE {\bfseries Input:} data $x_i$, size $m$
   \REPEAT
   \STATE Initialize $noChange = true$.
   \FOR{$i=1$ {\bfseries to} $m-1$}
   \IF{$x_i > x_{i+1}$}
   \STATE Swap $x_i$ and $x_{i+1}$
   \STATE $noChange = false$
   \ENDIF
   \ENDFOR
   \UNTIL{$noChange$ is $true$}
\end{algorithmic}
\end{algorithm}

\subsection{Tables}

You may also want to include tables that summarize material. Like
figures, these should be centered, legible, and numbered consecutively.
However, place the title \emph{above} the table with at least
0.1~inches of space before the title and the same after it, as in
\cref{sample-table}. The table title should be set in 9~point
type and centered unless it runs two or more lines, in which case it
should be flush left.

% Note use of \abovespace and \belowspace to get reasonable spacing
% above and below tabular lines.

\begin{table}[t]
\caption{Classification accuracies for naive Bayes and flexible
Bayes on various data sets.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Data set & Naive & Flexible & Better? \\
\midrule
Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

Tables contain textual material, whereas figures contain graphical material.
Specify the contents of each row and column in the table's topmost
row. Again, you may float tables to a column's top or bottom, and set
wide tables across both columns. Place two-column tables at the
top or bottom of the page.

\subsection{Theorems and such}
The preferred way is to number definitions, propositions, lemmas, etc. consecutively, within sections, as shown below.
\begin{definition}
\label{def:inj}
A function $f:X \to Y$ is injective if for any $x,y\in X$ different, $f(x)\ne f(y)$.
\end{definition}
Using \cref{def:inj} we immediate get the following result:
\begin{proposition}
If $f$ is injective mapping a set $X$ to another set $Y$, 
the cardinality of $Y$ is at least as large as that of $X$
\end{proposition}
\begin{proof} 
Left as an exercise to the reader. 
\end{proof}
\cref{lem:usefullemma} stated next will prove to be useful.
\begin{lemma}
\label{lem:usefullemma}
For any $f:X \to Y$ and $g:Y\to Z$ injective functions, $f \circ g$ is injective.
\end{lemma}
\begin{theorem}
\label{thm:bigtheorem}
If $f:X\to Y$ is bijective, the cardinality of $X$ and $Y$ are the same.
\end{theorem}
An easy corollary of \cref{thm:bigtheorem} is the following:
\begin{corollary}
If $f:X\to Y$ is bijective, 
the cardinality of $X$ is at least as large as that of $Y$.
\end{corollary}
\begin{assumption}
The set $X$ is finite.
\label{ass:xfinite}
\end{assumption}
\begin{remark}
According to some, it is only the finite case (cf. \cref{ass:xfinite}) that is interesting.
\end{remark}
%restatable

\subsection{Citations and References}

Please use APA reference format regardless of your formatter
or word processor. If you rely on the \LaTeX\/ bibliographic
facility, use \texttt{natbib.sty} and \texttt{icml2023.bst}
included in the style-file package to obtain this format.

Citations within the text should include the authors' last names and
year. If the authors' names are included in the sentence, place only
the year in parentheses, for example when referencing Arthur Samuel's
pioneering work \yrcite{Samuel59}. Otherwise place the entire
reference in parentheses with the authors and year separated by a
comma \cite{Samuel59}. List multiple references separated by
semicolons \cite{kearns89,Samuel59,mitchell80}. Use the `et~al.'
construct only for citations with three or more authors or after
listing all authors to a publication in an earlier reference \cite{MachineLearningI}.

Authors should cite their own work in the third person
in the initial version of their paper submitted for blind review.
Please refer to \cref{author info} for detailed instructions on how to
cite your own papers.

Use an unnumbered first-level section heading for the references, and use a
hanging indent style, with the first line of the reference flush against the
left margin and subsequent lines indented by 10 points. The references at the
end of this document give examples for journal articles \cite{Samuel59},
conference publications \cite{langley00}, book chapters \cite{Newell81}, books
\cite{DudaHart2nd}, edited volumes \cite{MachineLearningI}, technical reports
\cite{mitchell80}, and dissertations \cite{kearns89}.

Alphabetize references by the surnames of the first authors, with
single author entries preceding multiple author entries. Order
references for the same authors by year of publication, with the
earliest first. Make sure that each reference includes all relevant
information (e.g., page numbers).

Please put some effort into making references complete, presentable, and
consistent, e.g. use the actual current name of authors.
If using bibtex, please protect capital letters of names and
abbreviations in titles, for example, use \{B\}ayesian or \{L\}ipschitz
in your .bib file.
